Change Detection in Multivariate data streams: Online Analysis with Kernel-QuantTree

We present Kernel-QuantTree Exponentially Weighted Moving Average (KQT-EWMA), a non-parametric change-detection algorithm that combines the Kernel-QuantTree (KQT) histogram and the EWMA statistic to monitor multivariate data streams online. The resulting monitoring scheme is very flexible, since histograms can be used to model any stationary distribution, and practical, since the distribution of test statistics does not depend on the distribution of datastream in stationary conditions (non-parametric monitoring). KQT-EWMA enables controlling false alarms by operating at a pre-determined Average Run Length ($ARL_0$), which measures the expected number of stationary samples to be monitored before triggering a false alarm. The latter peculiarity is in contrast with most non-parametric change-detection tests, which rarely can control the $ARL_0$ a priori. Our experiments on synthetic and real-world datasets demonstrate that KQT-EWMA can control $ARL_0$ while achieving detection delays comparable to or lower than state-of-the-art methods designed to work in the same conditions.

==> tikz/plots/target_empirical_arl0.tex <==
\begin{tikzpicture}
\begin{groupplot}[
    % % % % These options are valid for ALL the plots in the groupplot
    %% GROUP OPTIONS
    group style={group size=4 by 2, vertical sep=1.8cm, horizontal sep=.6cm}, % vertical sep=1.5cm, horizontal sep=.15cm
    width=.21\textwidth,
    height=.18\textwidth,
    %% TITLE OPTIONS
    % title style = {font=\small, at={(0.5, 0.82)}, },
    title style = {font=\small, align=center},
    scale only axis, % (I've always seen this but have no idea what it does)
    % AXIS LABELS
    xlabel style = {font=\small},
    ylabel style = {font=\small},
    % TICKS (and their labels)
    % xtick = {0,2,...,12}, % the ... means "keep the same increment until you reach..."
    % minor xtick = {0.5,1.0,...,10.5},  % this sets the minor xticks
    % xticklabel style = {font = \scriptsize},
    % ytick = {.0,.2,...,1.0},
    ymajorgrids,    % set the grid lines on major y ticks
    xmajorgrids,
    xticklabel style = {font = \scriptsize, rotate=90},
    yticklabel style = {font = \scriptsize},
    % yticklabel = \empty,
    % xticklabel = \empty,
    % xtick = {,,},
    % ytick = {,,},
    %% AXIS LIMITS
    % xmin=-.02,
    % xmax=10.1,
    % ymin=0.2,
    % ymax=1.02
]
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % PLOT 1 - N = 128 % % % %
\nextgroupplot[
    title={$N=128$},
    xlabel={Target $ARL_0$},
    ylabel={Empirical $ARL_0$},
    xtick = {500, 1000, 2000, 5000},
    ytick = {500, 1000, 2000, 5000},
    legend style={
        at={($(0,0)+(0cm,0cm)$)},
        legend columns=3,
        fill=none,
        draw=black,
        anchor=center,
        align=center,
        font=\small,
        legend to name = arl_legend,
        },
]
\addplot[StyKQTEWMAL2] table[x=target, y=KQTEWMA-L2]
{tikz/data/arl0_N128.txt};
\addlegendentry{KQT-EWMA-l2}
%
\addplot[StyKQTEWMAMaha] table[x=target, y=KQTEWMA-Maha]
{tikz/data/arl0_N128.txt};
\addlegendentry{KQT-EWMA-maha}
%
\addplot[StyKQTEWMAWM] table[x=target, y=KQTEWMA-WM]
{tikz/data/arl0_N128.txt};
\addlegendentry{KQT-EWMA-weight}
%
\addplot[StyQTEWMA] table[x=target, y=QTEWMA]
{tikz/data/arl0_N128.txt};
\addlegendentry{QT-EWMA}
%
\addplot[StySPLL] table[x=target, y=SPLL]
{tikz/data/arl0_N128.txt};
\addlegendentry{SPLL}
%
\addplot[StySPLLCPM] table[x=target, y=SPLL-CPM]
{tikz/data/arl0_N128.txt};
\addlegendentry{SPLL-CPM}
%
\addplot[StyScanB] table[x=target, y=ScanB]
{tikz/data/arl0_N128.txt};
\addlegendentry{Scan-B}
% Black line
\addplot[color=black, dashed, forget plot] table[x=target, y=perfect]
{tikz/data/arl0_N128.txt};
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % PLOT 2 - N = 256 % % % %
\nextgroupplot[title={$N=256$}, xlabel={Target $ARL_0$}, xtick = {500, 1000, 2000, 5000}]
\addplot[StyKQTEWMAL2] table[x=target, y=KQTEWMA-L2] {tikz/data/arl0_N128.txt};
\addplot[StyKQTEWMAMaha] table[x=target, y=KQTEWMA-Maha] {tikz/data/arl0_N128.txt};
\addplot[StyKQTEWMAWM] table[x=target, y=KQTEWMA-WM] {tikz/data/arl0_N128.txt};
\addplot[StyQTEWMA] table[x=target, y=QTEWMA] {tikz/data/arl0_N128.txt};
\addplot[StySPLL] table[x=target, y=SPLL] {tikz/data/arl0_N128.txt};
\addplot[StySPLLCPM] table[x=target, y=SPLL-CPM] {tikz/data/arl0_N128.txt};
\addplot[StyScanB] table[x=target, y=ScanB] {tikz/data/arl0_N128.txt};
\addplot[color=black, dashed, forget plot] table[x=target, y=perfect] {tikz/data/arl0_N128.txt};
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % PLOT 3 - N = 1024 % % % %
\nextgroupplot[title={$N=1024$}, xlabel={Target $ARL_0$}, xtick = {500, 1000, 2000, 5000}]
\addplot[StyKQTEWMAL2] table[x=target, y=KQTEWMA-L2] {tikz/data/arl0_N128.txt};
\addplot[StyKQTEWMAMaha] table[x=target, y=KQTEWMA-Maha] {tikz/data/arl0_N128.txt};
\addplot[StyKQTEWMAWM] table[x=target, y=KQTEWMA-WM] {tikz/data/arl0_N128.txt};
\addplot[StyQTEWMA] table[x=target, y=QTEWMA] {tikz/data/arl0_N128.txt};
\addplot[StySPLL] table[x=target, y=SPLL] {tikz/data/arl0_N128.txt};
\addplot[StySPLLCPM] table[x=target, y=SPLL-CPM] {tikz/data/arl0_N128.txt};
\addplot[StyScanB] table[x=target, y=ScanB] {tikz/data/arl0_N128.txt};
\addplot[color=black, dashed, forget plot] table[x=target, y=perfect] {tikz/data/arl0_N128.txt};
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % PLOT 4 - N = 4096 % % % %
\nextgroupplot[title={$N=4096$}, xlabel={Target $ARL_0$}, xtick = {500, 1000, 2000, 5000}]
\addplot[StyKQTEWMAL2] table[x=target, y=KQTEWMA-L2] {tikz/data/arl0_N128.txt};
\addplot[StyKQTEWMAMaha] table[x=target, y=KQTEWMA-Maha] {tikz/data/arl0_N128.txt};
\addplot[StyKQTEWMAWM] table[x=target, y=KQTEWMA-WM] {tikz/data/arl0_N128.txt};
\addplot[StyQTEWMA] table[x=target, y=QTEWMA] {tikz/data/arl0_N128.txt};
\addplot[StySPLL] table[x=target, y=SPLL] {tikz/data/arl0_N128.txt};
\addplot[StySPLLCPM] table[x=target, y=SPLL-CPM] {tikz/data/arl0_N128.txt};
\addplot[StyScanB] table[x=target, y=ScanB] {tikz/data/arl0_N128.txt};
\addplot[color=black, dashed, forget plot] table[x=target, y=perfect] {tikz/data/arl0_N128.txt};
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%% SECOND ROW %%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % PLOT 5 - N = 128 % % % %
\nextgroupplot[xlabel={FA Rate}, ylabel={Detection Delay}, xtick = {0.06, 0.14, 0.26, 0.45}, ytick = {100, 1000}, xticklabel style={/pgf/number format/fixed, /pgf/number format/precision=2}]
\addplot[StyKQTEWMAL2] table[x=farate, y=KQTEWMA-L2] {tikz/data/delay_N128.txt};
\addplot[StyKQTEWMAMaha] table[x=farate, y=KQTEWMA-Maha] {tikz/data/delay_N128.txt};
\addplot[StyKQTEWMAWM] table[x=farate, y=KQTEWMA-WM] {tikz/data/delay_N128.txt};
\addplot[StyQTEWMA] table[x=farate, y=QTEWMA] {tikz/data/delay_N128.txt};
\addplot[StySPLL] table[x=farate, y=SPLL] {tikz/data/delay_N128.txt};
\addplot[StySPLLCPM] table[x=farate, y=SPLL-CPM] {tikz/data/delay_N128.txt};
\addplot[StyScanB] table[x=farate, y=ScanB] {tikz/data/delay_N128.txt};
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % PLOT 6 - N = 256 % % % %
\nextgroupplot[xlabel={FA Rate}, xtick = {0.06, 0.14, 0.26, 0.45}, xticklabel style={/pgf/number format/fixed, /pgf/number format/precision=2}]
\addplot[StyKQTEWMAL2] table[x=farate, y=KQTEWMA-L2] {tikz/data/delay_N128.txt};
\addplot[StyKQTEWMAMaha] table[x=farate, y=KQTEWMA-Maha] {tikz/data/delay_N128.txt};
\addplot[StyKQTEWMAWM] table[x=farate, y=KQTEWMA-WM] {tikz/data/delay_N128.txt};
\addplot[StyQTEWMA] table[x=farate, y=QTEWMA] {tikz/data/delay_N128.txt};
\addplot[StySPLL] table[x=farate, y=SPLL] {tikz/data/delay_N128.txt};
\addplot[StySPLLCPM] table[x=farate, y=SPLL-CPM] {tikz/data/delay_N128.txt};
\addplot[StyScanB] table[x=farate, y=ScanB] {tikz/data/delay_N128.txt};
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % PLOT 7 - N = 1024 % % % %
\nextgroupplot[xlabel={FA Rate}, xtick = {0.06, 0.14, 0.26, 0.45}, xticklabel style={/pgf/number format/fixed, /pgf/number format/precision=2}]
\addplot[StyKQTEWMAL2] table[x=farate, y=KQTEWMA-L2] {tikz/data/delay_N128.txt};
\addplot[StyKQTEWMAMaha] table[x=farate, y=KQTEWMA-Maha] {tikz/data/delay_N128.txt};
\addplot[StyKQTEWMAWM] table[x=farate, y=KQTEWMA-WM] {tikz/data/delay_N128.txt};
\addplot[StyQTEWMA] table[x=farate, y=QTEWMA] {tikz/data/delay_N128.txt};
\addplot[StySPLL] table[x=farate, y=SPLL] {tikz/data/delay_N128.txt};
\addplot[StySPLLCPM] table[x=farate, y=SPLL-CPM] {tikz/data/delay_N128.txt};
\addplot[StyScanB] table[x=farate, y=ScanB] {tikz/data/delay_N128.txt};
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % % % PLOT 8 - N = 4096 % % % %
\nextgroupplot[xlabel={FA Rate}, xtick = {0.06, 0.14, 0.26, 0.45}, xticklabel style={/pgf/number format/fixed, /pgf/number format/precision=2}]
\addplot[StyKQTEWMAL2] table[x=farate, y=KQTEWMA-L2] {tikz/data/delay_N128.txt};
\addplot[StyKQTEWMAMaha] table[x=farate, y=KQTEWMA-Maha] {tikz/data/delay_N128.txt};
\addplot[StyKQTEWMAWM] table[x=farate, y=KQTEWMA-WM] {tikz/data/delay_N128.txt};
\addplot[StyQTEWMA] table[x=farate, y=QTEWMA] {tikz/data/delay_N128.txt};
\addplot[StySPLL] table[x=farate, y=SPLL] {tikz/data/delay_N128.txt};
\addplot[StySPLLCPM] table[x=farate, y=SPLL-CPM] {tikz/data/delay_N128.txt};
\addplot[StyScanB] table[x=farate, y=ScanB] {tikz/data/delay_N128.txt};
%
\end{groupplot}
%
\node at ($(group c1r2)!.5!(group c4r2) + (0cm,-3.2cm)$) {\ref{arl_legend}};
% \node[text width=1cm] at ($(group c1r1) + (0.3cm,-2cm)$) {(a)};
% \node[text width=1cm] at ($(group c2r1) + (0.3cm,-2cm)$) {(b)};
%\node[text width=1cm] at ($(group c1r2) + (-3cm,2.2cm)$) {(b)}
% \node[text width=1cm] at ($(group c2r1) + (-3cm,2.2cm)$) {(c)}
% \node[text width=1cm] at ($(group c2r2) + (-3cm,2.2cm)$) {(d)}
%
\end{tikzpicture}%
% \node[text width=1cm] at (8, -4) {(a)}; % Node can be use to add text to the plot
